Beyond temperature scaling: Obtaining well-calibrated multiclass probabilities with Dirichlet calibration

Class probabilities predicted by most multiclass classifiers are uncalibrated, often tending towards over-confidence. With neural networks, calibration can be improved by temperature scaling, a method to learn a single corrective multiplicative factor for inputs to the last softmax layer. On non-neural models the existing methods apply binary calibration in a pairwise or one-vs-rest fashion. We propose a natively multiclass calibration method applicable to classifiers from any model class, derived from Dirichlet distributions and generalising the beta calibration method from binary classification. It is easily implemented with neural nets since it is equivalent to log-transforming the uncalibrated probabilities, followed by one linear layer and softmax. Experiments demonstrate improved probabilistic predictions according to multiple measures (confidence-ECE, classwise-ECE, log-loss, Brier score) across a wide range of datasets and classifiers. Parameters of the learned Dirichlet calibration map provide insights to the biases in the uncalibrated model.

==> tables/results/acc_rankings.tex <==
\begin{table}[tph]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{2.5}$ & $4.1$ & $2.9$ & $4.5$ & $3.1$ & $5.3$ & $5.5$\\
forest & $4.0$ & $\mathbf{3.0}$ & $5.6$ & $3.2$ & $4.4$ & $3.9$ & $3.9$\\
knn & $5.0$ & $3.9$ & $4.8$ & $\mathbf{3.1}$ & $3.1$ & $4.0$ & $4.0$\\
lda & $3.5$ & $5.1$ & $4.9$ & $3.7$ & $5.0$ & $3.0$ & $\mathbf{2.9}$\\
logistic & $\mathbf{2.1}$ & $3.7$ & $5.3$ & $4.0$ & $3.6$ & $4.6$ & $4.7$\\
mlp & $2.9$ & $\mathbf{2.8}$ & $5.9$ & $3.7$ & $4.5$ & $4.0$ & $4.3$\\
nbayes & $\mathbf{1.4}$ & $3.8$ & $3.0$ & $2.9$ & $5.0$ & $6.0$ & $6.0$\\
qda & $\mathbf{2.7}$ & $3.6$ & $3.9$ & $2.9$ & $3.8$ & $5.6$ & $5.6$\\
svc-linear & $\mathbf{1.8}$ & $3.5$ & $5.7$ & $2.8$ & $4.3$ & $5.1$ & $4.8$\\
svc-rbf & $3.3$ & $3.5$ & $3.8$ & $\mathbf{3.2}$ & $3.6$ & $5.0$ & $5.5$\\
tree & $3.7$ & $4.8$ & $4.5$ & $5.0$ & $4.3$ & $2.8$ & $2.8$\\
\midrule
avg rank & \bf{2.99} & 3.78 & 4.58 & 3.55 & 4.07 & 4.48 & 4.54\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=acc}
\label{table:acc}
\end{table}

==> tables/results/adas_dataset_vs_method_conf-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $0.06_{3}$ & $0.08_{5}$ & $0.05_{2}$ & $\mathbf{0.05_{1}}$ & $0.07_{4}$ & $0.16_{6}$ & $0.20_{7}$\\
balance-sc & $\mathbf{0.04_{1}}$ & $0.10_{3}$ & $0.17_{4}$ & $0.09_{2}$ & $0.18_{5}$ & $0.48_{6}$ & $0.55_{7}$\\
car & $\mathbf{0.07_{1}}$ & $0.10_{4}$ & $0.12_{5}$ & $0.07_{2}$ & $0.09_{3}$ & $0.14_{7}$ & $0.14_{6}$\\
cleveland & $\mathbf{0.14_{1}}$ & $0.17_{3}$ & $0.20_{6}$ & $0.15_{2}$ & $0.20_{5}$ & $0.20_{4}$ & $0.23_{7}$\\
dermatolog & $\mathbf{0.16_{1}}$ & $0.17_{3}$ & $0.26_{5}$ & $0.17_{2}$ & $0.24_{4}$ & $0.37_{7}$ & $0.33_{6}$\\
glass & $0.12_{2}$ & $\mathbf{0.11_{1}}$ & $0.16_{5}$ & $0.14_{3}$ & $0.14_{4}$ & $0.24_{7}$ & $0.21_{6}$\\
iris & $0.07_{4}$ & $\mathbf{0.05_{1}}$ & $0.17_{7}$ & $0.06_{2}$ & $0.11_{6}$ & $0.09_{5}$ & $0.07_{3}$\\
landsat-sa & $\mathbf{0.10_{1}}$ & $0.21_{4}$ & $0.18_{2}$ & $0.21_{5}$ & $0.21_{3}$ & $0.28_{6}$ & $0.33_{7}$\\
libras-mov & $0.08_{2}$ & $\mathbf{0.07_{1}}$ & $0.10_{5}$ & $0.09_{3}$ & $0.10_{6}$ & $0.10_{7}$ & $0.09_{4}$\\
mfeat-karh & $0.16_{3}$ & $0.15_{2}$ & $0.19_{5}$ & $\mathbf{0.14_{1}}$ & $0.18_{4}$ & $0.24_{6}$ & $0.24_{7}$\\
mfeat-morp & $\mathbf{0.14_{1}}$ & $0.14_{2}$ & $0.16_{4}$ & $0.16_{5}$ & $0.16_{3}$ & $0.24_{7}$ & $0.24_{6}$\\
mfeat-zern & $\mathbf{0.14_{1}}$ & $0.17_{4}$ & $0.17_{3}$ & $0.15_{2}$ & $0.18_{5}$ & $0.29_{6}$ & $0.29_{7}$\\
optdigits & $\mathbf{0.22_{1}}$ & $0.32_{4}$ & $0.31_{3}$ & $0.31_{2}$ & $0.33_{5}$ & $0.44_{6}$ & $0.46_{7}$\\
page-block & $\mathbf{0.03_{1}}$ & $0.06_{4}$ & $0.05_{3}$ & $0.22_{5}$ & $0.04_{2}$ & $0.56_{6}$ & $0.64_{7}$\\
pendigits & $0.13_{3}$ & $\mathbf{0.13_{1}}$ & $0.14_{5}$ & $0.13_{2}$ & $0.14_{4}$ & $0.22_{6}$ & $0.24_{7}$\\
segment & $0.05_{2}$ & $\mathbf{0.05_{1}}$ & $0.08_{4}$ & $0.08_{5}$ & $0.06_{3}$ & $0.09_{6}$ & $0.10_{7}$\\
vehicle & $\mathbf{0.08_{1}}$ & $0.09_{3}$ & $0.12_{5}$ & $0.08_{2}$ & $0.12_{4}$ & $0.14_{6}$ & $0.27_{7}$\\
vowel & $0.07_{3}$ & $0.07_{2}$ & $0.09_{5}$ & $\mathbf{0.07_{1}}$ & $0.09_{4}$ & $0.10_{7}$ & $0.10_{6}$\\
waveform-5 & $\mathbf{0.03_{1}}$ & $0.04_{4}$ & $0.06_{5}$ & $0.04_{2}$ & $0.06_{6}$ & $0.04_{3}$ & $0.41_{7}$\\
yeast & $\mathbf{0.06_{1}}$ & $0.07_{2}$ & $0.08_{3}$ & $0.15_{5}$ & $0.08_{4}$ & $0.26_{6}$ & $0.26_{7}$\\
\midrule
avg rank & \bf{1.70} & 2.70 & 4.30 & 2.70 & 4.20 & 6.00 & 6.40\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier adas with the measure=conf-ece(Friedman statistic test = 7.95E+01, p-value = 4.44E-15)}
\label{table:adas:conf-ece}
\end{table}


==> tables/results/adas_dataset_vs_method_cw-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $0.21_{5}$ & $0.25_{7}$ & $0.15_{3}$ & $0.14_{2}$ & $0.18_{4}$ & $0.23_{6}$ & $\mathbf{0.10_{1}}$\\
balance-sc & $\mathbf{0.10_{1}}$ & $0.22_{3}$ & $0.36_{4}$ & $0.20_{2}$ & $0.38_{5}$ & $0.89_{7}$ & $0.60_{6}$\\
car & $0.18_{2}$ & $0.23_{3}$ & $0.29_{5}$ & $\mathbf{0.18_{1}}$ & $0.25_{4}$ & $0.32_{7}$ & $0.29_{6}$\\
cleveland & $\mathbf{0.41_{1}}$ & $0.41_{3}$ & $0.44_{4}$ & $0.41_{2}$ & $0.45_{5}$ & $0.54_{6}$ & $0.58_{7}$\\
dermatolog & $\mathbf{0.41_{1}}$ & $0.43_{2}$ & $0.64_{5}$ & $0.44_{3}$ & $0.57_{4}$ & $0.79_{7}$ & $0.72_{6}$\\
glass & $0.39_{2}$ & $\mathbf{0.38_{1}}$ & $0.49_{5}$ & $0.48_{4}$ & $0.44_{3}$ & $0.79_{7}$ & $0.75_{6}$\\
iris & $0.15_{4}$ & $\mathbf{0.13_{1}}$ & $0.36_{7}$ & $0.13_{2}$ & $0.24_{6}$ & $0.18_{5}$ & $0.14_{3}$\\
landsat-sa & $\mathbf{0.25_{1}}$ & $0.55_{4}$ & $0.43_{2}$ & $0.56_{5}$ & $0.50_{3}$ & $0.70_{6}$ & $0.76_{7}$\\
libras-mov & $0.51_{2}$ & $0.52_{3}$ & $0.57_{7}$ & $0.56_{6}$ & $0.55_{5}$ & $0.53_{4}$ & $\mathbf{0.51_{1}}$\\
mfeat-karh & $0.48_{4}$ & $0.47_{3}$ & $0.51_{6}$ & $0.61_{7}$ & $0.49_{5}$ & $\mathbf{0.32_{1}}$ & $0.40_{2}$\\
mfeat-morp & $\mathbf{0.41_{1}}$ & $0.42_{2}$ & $0.46_{3}$ & $0.53_{5}$ & $0.47_{4}$ & $0.62_{6}$ & $0.63_{7}$\\
mfeat-zern & $0.44_{3}$ & $0.51_{5}$ & $0.51_{4}$ & $0.60_{7}$ & $0.53_{6}$ & $\mathbf{0.32_{1}}$ & $0.32_{2}$\\
optdigits & $\mathbf{0.50_{1}}$ & $0.75_{6}$ & $0.68_{4}$ & $0.80_{7}$ & $0.74_{5}$ & $0.56_{3}$ & $0.51_{2}$\\
page-block & $\mathbf{0.07_{1}}$ & $0.13_{4}$ & $0.10_{3}$ & $0.45_{5}$ & $0.09_{2}$ & $1.15_{6}$ & $1.30_{7}$\\
pendigits & $0.38_{2}$ & $0.41_{6}$ & $0.40_{4}$ & $0.57_{7}$ & $0.40_{3}$ & $\mathbf{0.27_{1}}$ & $0.41_{5}$\\
segment & $0.16_{2}$ & $\mathbf{0.15_{1}}$ & $0.22_{4}$ & $0.24_{5}$ & $0.18_{3}$ & $0.26_{6}$ & $0.29_{7}$\\
vehicle & $\mathbf{0.23_{1}}$ & $0.26_{3}$ & $0.35_{5}$ & $0.25_{2}$ & $0.32_{4}$ & $0.49_{6}$ & $0.66_{7}$\\
vowel & $0.23_{3}$ & $0.22_{2}$ & $0.25_{4}$ & $0.30_{7}$ & $\mathbf{0.21_{1}}$ & $0.26_{5}$ & $0.27_{6}$\\
waveform-5 & $\mathbf{0.08_{1}}$ & $0.10_{3}$ & $0.13_{5}$ & $0.09_{2}$ & $0.14_{6}$ & $0.11_{4}$ & $0.73_{7}$\\
yeast & $\mathbf{0.24_{1}}$ & $0.26_{2}$ & $0.26_{3}$ & $0.64_{5}$ & $0.31_{4}$ & $0.87_{6}$ & $0.89_{7}$\\
\midrule
avg rank & \bf{1.95} & 3.20 & 4.35 & 4.30 & 4.10 & 5.00 & 5.10\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier adas with the measure=cw-ece(Friedman statistic test = 3.12E+01, p-value = 2.34E-05)}
\label{table:adas:cw-ece}
\end{table}


==> tables/results/adas_dataset_vs_method_p-conf-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $0.06_{3}$ & $0.00_{5}$ & $0.09_{2}$ & $\mathbf{0.12_{1}}$ & $0.01_{4}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
balance-sc & $\mathbf{0.44_{1}}$ & $0.02_{3}$ & $0.00_{4}$ & $0.02_{2}$ & $0.00_{5}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
car & $0.12_{2}$ & $0.03_{4}$ & $0.00_{5}$ & $\mathbf{0.13_{1}}$ & $0.06_{3}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
cleveland & $\mathbf{0.56_{1}}$ & $0.33_{3}$ & $0.08_{6}$ & $0.46_{2}$ & $0.13_{4}$ & $0.09_{5}$ & $0.03_{7}$\\
dermatolog & $\mathbf{0.09_{1}}$ & $0.08_{2}$ & $0.01_{5}$ & $0.07_{3}$ & $0.03_{4}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
glass & $0.55_{2}$ & $\mathbf{0.55_{1}}$ & $0.27_{5}$ & $0.45_{3}$ & $0.35_{4}$ & $0.05_{7}$ & $0.12_{6}$\\
iris & $0.38_{2}$ & $\mathbf{0.47_{1}}$ & $0.11_{7}$ & $0.36_{3}$ & $0.24_{6}$ & $0.36_{4}$ & $0.29_{5}$\\
landsat-sa & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$\\
libras-mov & $0.37_{2}$ & $\mathbf{0.45_{1}}$ & $0.06_{6}$ & $0.30_{3}$ & $0.11_{5}$ & $0.06_{7}$ & $0.17_{4}$\\
mfeat-karh & $\mathbf{0.01_{1}}$ & $0.00_{2}$ & $0.00_{4}$ & $0.00_{3}$ & $0.00_{5}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
mfeat-morp & $0.05_{2}$ & $\mathbf{0.06_{1}}$ & $0.03_{4}$ & $0.00_{5}$ & $0.04_{3}$ & $0.00_{7}$ & $0.00_{6}$\\
mfeat-zern & $\mathbf{0.00_{1}}$ & $0.00_{5}$ & $0.00_{5}$ & $0.00_{2}$ & $0.00_{5}$ & $0.00_{5}$ & $0.00_{5}$\\
optdigits & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$\\
page-block & $\mathbf{0.06_{1}}$ & $0.00_{4}$ & $0.00_{3}$ & $0.00_{6}$ & $0.02_{2}$ & $0.00_{6}$ & $0.00_{6}$\\
pendigits & $0.00_{2.5}$ & $0.00_{5.5}$ & $\mathbf{0.00_{1}}$ & $0.00_{2.5}$ & $0.00_{5.5}$ & $0.00_{5.5}$ & $0.00_{5.5}$\\
segment & $\mathbf{0.24_{1}}$ & $0.24_{2}$ & $0.10_{6}$ & $0.04_{7}$ & $0.17_{4}$ & $0.19_{3}$ & $0.13_{5}$\\
vehicle & $0.34_{3}$ & $0.35_{2}$ & $0.09_{4}$ & $\mathbf{0.40_{1}}$ & $0.09_{5}$ & $0.05_{6}$ & $0.00_{7}$\\
vowel & $\mathbf{0.33_{1}}$ & $0.30_{2}$ & $0.19_{5}$ & $0.23_{3}$ & $0.17_{6}$ & $0.14_{7}$ & $0.20_{4}$\\
waveform-5 & $\mathbf{0.37_{1}}$ & $0.08_{4}$ & $0.00_{5}$ & $0.15_{2}$ & $0.00_{6}$ & $0.09_{3}$ & $0.00_{7}$\\
yeast & $\mathbf{0.28_{1}}$ & $0.11_{3}$ & $0.19_{2}$ & $0.00_{5}$ & $0.08_{4}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
\midrule
avg rank & \bf{1.83} & 2.93 & 4.35 & 3.12 & 4.43 & 5.63 & 5.73\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier adas with the measure=p-conf-ece(Friedman statistic test = 6.24E+01, p-value = 1.46E-11)}
\label{table:adas:p-conf-ece}
\end{table}


==> tables/results/adas_dataset_vs_method_p-cw-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $0.00_{5}$ & $0.00_{6.5}$ & $0.05_{2}$ & $\mathbf{0.09_{1}}$ & $0.01_{4}$ & $0.00_{6.5}$ & $0.02_{3}$\\
balance-sc & $\mathbf{0.58_{1}}$ & $0.02_{3}$ & $0.00_{4}$ & $0.04_{2}$ & $0.00_{5}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
car & $0.07_{2}$ & $0.00_{4}$ & $0.00_{5}$ & $\mathbf{0.09_{1}}$ & $0.03_{3}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
cleveland & $0.49_{3}$ & $0.53_{2}$ & $0.35_{4}$ & $\mathbf{0.64_{1}}$ & $0.32_{5}$ & $0.11_{6}$ & $0.05_{7}$\\
dermatolog & $0.08_{2}$ & $\mathbf{0.08_{1}}$ & $0.01_{5}$ & $0.05_{3}$ & $0.03_{4}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
glass & $\mathbf{0.64_{1}}$ & $0.61_{2}$ & $0.36_{4}$ & $0.28_{5}$ & $0.50_{3}$ & $0.00_{7}$ & $0.01_{6}$\\
iris & $\mathbf{0.44_{1}}$ & $0.43_{2}$ & $0.22_{7}$ & $0.38_{5}$ & $0.39_{4}$ & $0.42_{3}$ & $0.29_{6}$\\
landsat-sa & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$\\
libras-mov & $0.55_{2}$ & $\mathbf{0.61_{1}}$ & $0.30_{5}$ & $0.25_{7}$ & $0.34_{4}$ & $0.29_{6}$ & $0.46_{3}$\\
mfeat-karh & $0.01_{2}$ & $0.00_{5}$ & $0.00_{4}$ & $0.00_{7}$ & $0.00_{6}$ & $\mathbf{0.02_{1}}$ & $0.00_{3}$\\
mfeat-morp & $\mathbf{0.06_{1}}$ & $0.04_{3}$ & $0.05_{2}$ & $0.00_{6}$ & $0.04_{4}$ & $0.00_{6}$ & $0.00_{6}$\\
mfeat-zern & $0.00_{3}$ & $0.00_{5.5}$ & $0.00_{5.5}$ & $0.00_{5.5}$ & $0.00_{5.5}$ & $\mathbf{0.06_{1}}$ & $0.01_{2}$\\
optdigits & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$\\
page-block & $0.03_{2}$ & $0.00_{5.5}$ & $0.02_{3}$ & $0.00_{5.5}$ & $\mathbf{0.03_{1}}$ & $0.00_{5.5}$ & $0.00_{5.5}$\\
pendigits & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$ & $0.00_{4}$\\
segment & $0.24_{2}$ & $\mathbf{0.24_{1}}$ & $0.23_{5}$ & $0.04_{7}$ & $0.24_{3}$ & $0.24_{4}$ & $0.23_{6}$\\
vehicle & $\mathbf{0.45_{1}}$ & $0.33_{3}$ & $0.03_{5}$ & $0.39_{2}$ & $0.10_{4}$ & $0.00_{6.5}$ & $0.00_{6.5}$\\
vowel & $0.50_{4}$ & $0.56_{2}$ & $0.51_{3}$ & $0.32_{7}$ & $\mathbf{0.66_{1}}$ & $0.40_{6}$ & $0.43_{5}$\\
waveform-5 & $\mathbf{0.42_{1}}$ & $0.13_{3}$ & $0.00_{5}$ & $0.20_{2}$ & $0.00_{6}$ & $0.06_{4}$ & $0.00_{7}$\\
yeast & $0.25_{2}$ & $0.07_{3}$ & $\mathbf{0.26_{1}}$ & $0.00_{6}$ & $0.06_{4}$ & $0.00_{6}$ & $0.00_{6}$\\
\midrule
avg rank & \bf{2.35} & 3.23 & 4.08 & 4.25 & 3.92 & 5.00 & 5.17\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier adas with the measure=p-cw-ece(Friedman statistic test = 3.02E+01, p-value = 3.64E-05)}
\label{table:adas:p-cw-ece}
\end{table}


==> tables/results/brier_rankings.tex <==
\begin{table}[tph]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{1.6}$ & $3.0$ & $3.3$ & $3.6$ & $3.6$ & $6.3$ & $6.5$\\
forest & $4.4$ & $\mathbf{1.8}$ & $5.4$ & $1.9$ & $3.9$ & $5.3$ & $5.3$\\
knn & $3.9$ & $3.5$ & $5.3$ & $\mathbf{1.9}$ & $3.8$ & $4.8$ & $4.8$\\
lda & $\mathbf{1.8}$ & $3.2$ & $5.3$ & $2.2$ & $3.9$ & $6.0$ & $5.8$\\
logistic & $\mathbf{1.6}$ & $2.7$ & $6.1$ & $2.5$ & $4.3$ & $4.3$ & $6.4$\\
mlp & $3.0$ & $\mathbf{2.2}$ & $6.6$ & $2.8$ & $5.2$ & $3.9$ & $4.2$\\
nbayes & $\mathbf{1.2}$ & $3.5$ & $4.2$ & $2.3$ & $4.9$ & $5.7$ & $6.2$\\
qda & $\mathbf{1.9}$ & $2.9$ & $5.8$ & $2.1$ & $4.4$ & $5.1$ & $5.7$\\
svc-linear & $\mathbf{1.5}$ & $2.8$ & $6.5$ & $2.6$ & $4.6$ & $4.1$ & $5.8$\\
svc-rbf & $3.0$ & $\mathbf{2.5}$ & $4.7$ & $2.8$ & $4.7$ & $4.5$ & $5.8$\\
tree & $3.4$ & $4.2$ & $6.5$ & $4.7$ & $5.4$ & $\mathbf{1.9}$ & $2.0$\\
\midrule
avg rank & \bf{2.48} & 2.94 & 5.43 & 2.67 & 4.43 & 4.72 & 5.33\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=brier}
\label{table:brier}
\end{table}

==> tables/results/conf-ece_rankings.tex <==
\begin{table}[tph]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{1.7}$ & $2.7$ & $4.3$ & $2.7$ & $4.2$ & $6.0$ & $6.4$\\
forest & $4.2$ & $2.2$ & $5.7$ & $\mathbf{1.4}$ & $4.4$ & $5.1$ & $5.1$\\
knn & $3.0$ & $\mathbf{3.0}$ & $6.1$ & $3.5$ & $5.8$ & $3.3$ & $3.3$\\
lda & $\mathbf{2.0}$ & $2.9$ & $5.9$ & $2.1$ & $4.0$ & $5.7$ & $5.5$\\
logistic & $2.2$ & $3.0$ & $6.3$ & $\mathbf{1.9}$ & $4.7$ & $3.8$ & $6.1$\\
mlp & $3.5$ & $2.7$ & $6.6$ & $\mathbf{1.4}$ & $5.7$ & $4.0$ & $4.2$\\
nbayes & $\mathbf{2.1}$ & $2.8$ & $5.2$ & $2.4$ & $4.3$ & $5.3$ & $5.9$\\
qda & $3.1$ & $2.3$ & $6.5$ & $\mathbf{1.7}$ & $4.7$ & $4.6$ & $5.1$\\
svc-linear & $2.7$ & $2.8$ & $6.7$ & $\mathbf{2.0}$ & $4.9$ & $3.4$ & $5.5$\\
svc-rbf & $3.7$ & $3.4$ & $6.5$ & $2.9$ & $4.5$ & $\mathbf{2.7}$ & $4.3$\\
tree & $2.6$ & $3.6$ & $6.8$ & $4.8$ & $5.7$ & $\mathbf{2.2}$ & $2.3$\\
\midrule
avg rank & 2.80 & 2.86 & 6.05 & \bf{2.42} & 4.81 & 4.17 & 4.89\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=conf-ece}
\label{table:conf-ece}
\end{table}

==> tables/results/cw-ece_rankings.tex <==
\begin{table}[tph]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{1.9}$ & $3.2$ & $4.3$ & $4.3$ & $4.1$ & $5.0$ & $5.1$\\
forest & $4.0$ & $2.1$ & $5.8$ & $\mathbf{1.1}$ & $4.0$ & $5.5$ & $5.4$\\
knn & $4.0$ & $3.9$ & $6.0$ & $3.6$ & $5.6$ & $2.5$ & $2.5$\\
lda & $2.4$ & $2.8$ & $5.8$ & $\mathbf{2.0}$ & $4.1$ & $5.3$ & $5.7$\\
logistic & $2.2$ & $2.5$ & $6.2$ & $\mathbf{2.0}$ & $4.4$ & $4.5$ & $6.1$\\
mlp & $3.0$ & $2.3$ & $6.6$ & $\mathbf{1.7}$ & $5.5$ & $4.3$ & $4.5$\\
nbayes & $\mathbf{1.9}$ & $3.5$ & $5.0$ & $2.5$ & $4.0$ & $5.4$ & $5.7$\\
qda & $2.7$ & $2.6$ & $6.4$ & $\mathbf{1.8}$ & $4.6$ & $5.0$ & $4.9$\\
svc-linear & $2.5$ & $2.6$ & $6.7$ & $\mathbf{2.5}$ & $4.6$ & $3.6$ & $5.5$\\
svc-rbf & $\mathbf{2.7}$ & $2.9$ & $6.5$ & $3.1$ & $4.5$ & $3.6$ & $4.7$\\
tree & $3.1$ & $4.1$ & $6.5$ & $4.7$ & $5.5$ & $\mathbf{1.9}$ & $2.0$\\
\midrule
avg rank & 2.76 & 2.95 & 5.97 & \bf{2.67} & 4.65 & 4.25 & 4.75\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=cw-ece}
\label{table:cw-ece}
\end{table}

==> tables/results/datasets.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  n\_samples &  n\_features &  n\_classes \\
dataset             &            &             &            \\
\midrule
abalone             &       4177 &           8 &          3 \\
balance-scale       &        625 &           4 &          3 \\
car                 &       1728 &           6 &          4 \\
cleveland           &        297 &          13 &          5 \\
dermatology         &        358 &          34 &          6 \\
glass               &        214 &           9 &          6 \\
iris                &        150 &           4 &          3 \\
landsat-satellite   &       6435 &          36 &          6 \\
libras-movement     &        360 &          90 &         15 \\
mfeat-karhunen      &       2000 &          64 &         10 \\
mfeat-morphological &       2000 &           6 &         10 \\
mfeat-zernike       &       2000 &          47 &         10 \\
optdigits           &       5620 &          64 &         10 \\
page-blocks         &       5473 &          10 &          5 \\
pendigits           &      10992 &          16 &         10 \\
segment             &       2310 &          19 &          7 \\
shuttle             &     101500 &           9 &          7 \\
vehicle             &        846 &          18 &          4 \\
vowel               &        990 &          10 &         11 \\
waveform-5000       &       5000 &          40 &          3 \\
yeast               &       1484 &           8 &         10 \\
\bottomrule
\end{tabular}


==> tables/results/ece_rankings.tex <==
\begin{table}[htp]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{2.5_{1}}$ & $3.6_{3}$ & $5.1_{7}$ & $3.0_{2}$ & $4.8_{6}$ & $4.5_{5}$ & $4.5_{4}$\\
logistic & $2.3_{2}$ & $2.5_{3}$ & $6.3_{7}$ & $\mathbf{2.0_{1}}$ & $4.7_{5}$ & $3.9_{4}$ & $6.2_{6}$\\
mlp & $3.1_{3}$ & $2.8_{2}$ & $6.6_{7}$ & $\mathbf{1.6_{1}}$ & $5.7_{6}$ & $4.0_{4}$ & $4.2_{5}$\\
svm & $2.7_{3}$ & $2.4_{2}$ & $6.8_{7}$ & $\mathbf{1.9_{1}}$ & $5.3_{5.5}$ & $3.6_{4}$ & $5.3_{5.5}$\\
forest & $4.0_{3}$ & $1.9_{2}$ & $5.9_{7}$ & $\mathbf{1.4_{1}}$ & $4.5_{4}$ & $4.8_{5}$ & $5.7_{6}$\\
nbayes & $\mathbf{2.0_{1}}$ & $2.9_{3}$ & $5.2_{5}$ & $2.1_{2}$ & $4.3_{4}$ & $5.5_{6}$ & $6.0_{7}$\\
\midrule
avg rank & 2.78 & 2.66 & 5.97 & \bf{2.00} & 4.88 & 4.38 & 5.32\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=ece}
\label{table:ece}
\end{table}

==> tables/results/exec_time_rankings.tex <==
\begin{table}[tph]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $6.5$ & $5.2$ & $3.5$ & $1.9$ & $3.5$ & $6.3$ & $\mathbf{1.1}$\\
forest & $6.5$ & $5.0$ & $3.7$ & $1.9$ & $3.3$ & $6.5$ & $\mathbf{1.1}$\\
knn & $6.8$ & $5.0$ & $3.4$ & $1.9$ & $3.5$ & $6.2$ & $\mathbf{1.1}$\\
lda & $6.8$ & $5.0$ & $3.8$ & $2.0$ & $3.2$ & $6.2$ & $\mathbf{1.0}$\\
logistic & $6.7$ & $5.0$ & $3.7$ & $2.0$ & $3.3$ & $6.3$ & $\mathbf{1.0}$\\
mlp & $6.7$ & $5.1$ & $3.8$ & $2.0$ & $3.3$ & $6.1$ & $\mathbf{1.0}$\\
nbayes & $6.6$ & $5.0$ & $3.8$ & $2.0$ & $3.2$ & $6.3$ & $\mathbf{1.0}$\\
qda & $6.7$ & $5.1$ & $3.7$ & $2.0$ & $3.3$ & $6.2$ & $\mathbf{1.0}$\\
svc-linear & $6.6$ & $5.0$ & $3.6$ & $1.9$ & $3.4$ & $6.4$ & $\mathbf{1.1}$\\
svc-rbf & $6.7$ & $5.2$ & $3.6$ & $1.9$ & $3.5$ & $6.0$ & $\mathbf{1.1}$\\
tree & $6.8$ & $5.1$ & $3.6$ & $2.0$ & $3.4$ & $6.2$ & $\mathbf{1.0}$\\
\midrule
avg rank & 6.66 & 5.08 & 3.65 & 1.96 & 3.36 & 6.24 & \bf{1.05}\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=exec_time}
\label{table:exec_time}
\end{table}

==> tables/results/join_nbayes_logloss_all_logloss.tex <==
\begin{table}
\begin{minipage}[t]{.56\textwidth}
\captionof{table}{Ranking of calibration methods applied on the classifier nbayes with the measure=loss(Friedman statistic test = 7.38E+01, p-value = 6.71E-14)}
\label{table:nbayes:loss}
\tiny
\centering
\setlength{\tabcolsep}{.5em}
\begin{tabular}{lcccccc|c}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
abalone & $\mathbf{0.89_{1}}$ & $0.89_{4}$ & $0.89_{2}$ & $0.90_{5}$ & $0.92_{6}$ & $0.89_{3}$ & $1.95_{7}$\\
balance-sc & $\mathbf{0.21_{1}}$ & $0.30_{2}$ & $0.36_{5}$ & $0.32_{3}$ & $0.35_{4}$ & $0.41_{6}$ & $0.47_{7}$\\
car & $\mathbf{0.38_{1}}$ & $0.59_{4}$ & $0.56_{2}$ & $0.57_{3}$ & $0.67_{5}$ & $1.56_{6.5}$ & $1.56_{6.5}$\\
cleveland & $\mathbf{1.02_{1}}$ & $1.30_{4}$ & $1.12_{2}$ & $1.38_{5}$ & $1.14_{3}$ & $2.18_{6}$ & $2.49_{7}$\\
dermatolog & $\mathbf{0.20_{1}}$ & $0.41_{5}$ & $0.23_{2}$ & $0.39_{3}$ & $0.40_{4}$ & $2.51_{7}$ & $2.51_{6}$\\
glass & $\mathbf{1.11_{1}}$ & $1.50_{4}$ & $1.14_{3}$ & $1.64_{5}$ & $1.12_{2}$ & $3.14_{6.5}$ & $3.14_{6.5}$\\
iris & $\mathbf{0.11_{1}}$ & $0.26_{5}$ & $0.33_{6}$ & $0.34_{7}$ & $0.21_{4}$ & $0.13_{3}$ & $0.13_{2}$\\
landsat-sa & $\mathbf{0.36_{1}}$ & $0.56_{2}$ & $0.58_{4}$ & $0.58_{3}$ & $0.74_{5}$ & $3.87_{6.5}$ & $3.87_{6.5}$\\
libras-mov & $\mathbf{0.97_{1}}$ & $1.36_{2}$ & $1.67_{4}$ & $1.91_{5}$ & $1.45_{3}$ & $4.90_{6.5}$ & $4.90_{6.5}$\\
mfeat-karh & $\mathbf{0.20_{1}}$ & $0.22_{2}$ & $0.38_{6}$ & $0.38_{5}$ & $0.29_{4}$ & $0.23_{3}$ & $0.44_{7}$\\
mfeat-morp & $\mathbf{0.72_{1}}$ & $0.91_{5}$ & $0.82_{2}$ & $0.87_{3}$ & $0.88_{4}$ & $1.75_{6.5}$ & $1.75_{6.5}$\\
mfeat-zern & $\mathbf{0.59_{1}}$ & $0.71_{2}$ & $0.82_{4}$ & $0.84_{6}$ & $0.84_{5}$ & $0.77_{3}$ & $1.73_{7}$\\
optdigits & $0.45_{2}$ & $0.57_{4}$ & $0.47_{3}$ & $\mathbf{0.44_{1}}$ & $0.84_{5}$ & $3.14_{6}$ & $3.14_{7}$\\
page-block & $\mathbf{0.17_{1}}$ & $0.21_{4}$ & $0.20_{3}$ & $0.18_{2}$ & $0.21_{5}$ & $0.74_{6.5}$ & $0.74_{6.5}$\\
pendigits & $\mathbf{0.19_{1}}$ & $0.46_{3}$ & $0.48_{4}$ & $0.46_{2}$ & $0.58_{5}$ & $1.30_{6.5}$ & $1.30_{6.5}$\\
segment & $\mathbf{0.28_{1}}$ & $0.62_{5}$ & $0.46_{3}$ & $0.45_{2}$ & $0.56_{4}$ & $1.39_{6.5}$ & $1.39_{6.5}$\\
vehicle & $\mathbf{0.99_{1}}$ & $1.09_{3}$ & $1.05_{2}$ & $1.13_{5}$ & $1.10_{4}$ & $1.16_{6}$ & $2.30_{7}$\\
vowel & $\mathbf{0.54_{1}}$ & $0.81_{2}$ & $1.07_{6}$ & $1.08_{7}$ & $0.90_{5}$ & $0.85_{4}$ & $0.84_{3}$\\
waveform-5 & $\mathbf{0.33_{1}}$ & $0.37_{2}$ & $0.38_{3}$ & $0.38_{4}$ & $0.46_{6}$ & $0.43_{5}$ & $0.80_{7}$\\
yeast & $\mathbf{1.18_{1}}$ & $1.41_{4}$ & $1.31_{2}$ & $1.33_{3}$ & $1.43_{5}$ & $5.10_{6.5}$ & $5.10_{6.5}$\\
\midrule
avg rank & \bf{1.05} & 3.40 & 3.40 & 3.95 & 4.40 & 5.53 & 6.28\\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{.42\textwidth}
\normalsize
\captionof{table}{Ranking of calibration methods applied to each classifier with the measure=loss}
\label{table:loss}
\tiny
\centering
\setlength{\tabcolsep}{.4em}
\begin{tabular}{lcccccc|c}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{1.4}$ & $3.1$ & $3.2$ & $4.3$ & $3.5$ & $5.9$ & $6.6$\\
forest & $4.2$ & $\mathbf{1.9}$ & $4.7$ & $4.1$ & $2.9$ & $5.2$ & $5.2$\\
knn & $3.8$ & $4.8$ & $3.0$ & $\mathbf{1.6}$ & $2.0$ & $6.5$ & $6.5$\\
lda & $\mathbf{1.6}$ & $2.2$ & $5.2$ & $5.2$ & $3.5$ & $4.6$ & $5.7$\\
logistic & $\mathbf{1.3}$ & $2.1$ & $5.8$ & $6.1$ & $3.5$ & $3.6$ & $5.6$\\
mlp & $\mathbf{2.2}$ & $2.3$ & $6.5$ & $6.2$ & $4.7$ & $2.9$ & $3.4$\\
nbayes & $\mathbf{1.1}$ & $3.4$ & $3.4$ & $4.0$ & $4.4$ & $5.5$ & $6.3$\\
qda & $\mathbf{1.7}$ & $2.7$ & $5.6$ & $4.6$ & $3.4$ & $4.2$ & $5.8$\\
svc-linear & $\mathbf{1.3}$ & $2.3$ & $6.1$ & $6.1$ & $4.3$ & $3.0$ & $4.8$\\
svc-rbf & $2.6$ & $\mathbf{2.2}$ & $4.3$ & $4.8$ & $4.5$ & $4.0$ & $5.6$\\
tree & $3.9$ & $5.1$ & $3.4$ & $\mathbf{2.1}$ & $2.4$ & $5.6$ & $5.6$\\
\midrule
avg rank & \bf{2.25} & 2.92 & 4.66 & 4.48 & 3.54 & 4.61 & 5.54\\
\bottomrule
\end{tabular}
\end{minipage}
\end{table}


==> tables/results/loss_rankings.tex <==
\begin{table}[tph]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{1.4}$ & $3.1$ & $3.2$ & $4.3$ & $3.5$ & $5.9$ & $6.6$\\
forest & $4.2$ & $\mathbf{1.9}$ & $4.7$ & $4.1$ & $2.9$ & $5.2$ & $5.2$\\
knn & $3.8$ & $4.8$ & $3.0$ & $\mathbf{1.6}$ & $2.0$ & $6.5$ & $6.5$\\
lda & $\mathbf{1.6}$ & $2.2$ & $5.2$ & $5.2$ & $3.5$ & $4.6$ & $5.7$\\
logistic & $\mathbf{1.3}$ & $2.1$ & $5.8$ & $6.1$ & $3.5$ & $3.6$ & $5.6$\\
mlp & $\mathbf{2.2}$ & $2.3$ & $6.5$ & $6.2$ & $4.7$ & $2.9$ & $3.4$\\
nbayes & $\mathbf{1.1}$ & $3.4$ & $3.4$ & $4.0$ & $4.4$ & $5.5$ & $6.3$\\
qda & $\mathbf{1.7}$ & $2.7$ & $5.6$ & $4.6$ & $3.4$ & $4.2$ & $5.8$\\
svc-linear & $\mathbf{1.3}$ & $2.3$ & $6.1$ & $6.1$ & $4.3$ & $3.0$ & $4.8$\\
svc-rbf & $2.6$ & $\mathbf{2.2}$ & $4.3$ & $4.8$ & $4.5$ & $4.0$ & $5.6$\\
tree & $3.9$ & $5.1$ & $3.4$ & $\mathbf{2.1}$ & $2.4$ & $5.6$ & $5.6$\\
\midrule
avg rank & \bf{2.25} & 2.92 & 4.66 & 4.48 & 3.54 & 4.61 & 5.54\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=loss}
\label{table:loss}
\end{table}

==> tables/results/mce_rankings.tex <==
\begin{table}[tph]
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{3.0}$ & $3.4$ & $3.5$ & $3.4$ & $3.6$ & $5.3$ & $5.9$\\
forest & $4.2$ & $\mathbf{3.2}$ & $4.8$ & $3.8$ & $3.4$ & $4.1$ & $4.5$\\
knn & $4.2$ & $4.7$ & $4.2$ & $3.7$ & $\mathbf{3.3}$ & $4.0$ & $4.0$\\
lda & $\mathbf{2.0}$ & $3.2$ & $4.8$ & $4.5$ & $4.0$ & $5.0$ & $4.5$\\
logistic & $3.4$ & $3.8$ & $5.4$ & $4.8$ & $\mathbf{2.5}$ & $3.5$ & $4.7$\\
mlp & $3.2$ & $4.2$ & $4.7$ & $4.6$ & $\mathbf{3.0}$ & $3.7$ & $4.5$\\
nbayes & $\mathbf{2.6}$ & $3.0$ & $3.6$ & $3.0$ & $4.2$ & $5.6$ & $5.9$\\
qda & $3.2$ & $\mathbf{2.2}$ & $5.1$ & $3.7$ & $4.2$ & $4.2$ & $5.4$\\
svc-linear & $\mathbf{2.8}$ & $4.2$ & $5.5$ & $3.7$ & $3.5$ & $4.1$ & $4.2$\\
svc-rbf & $5.0$ & $4.6$ & $3.9$ & $3.5$ & $\mathbf{3.3}$ & $3.5$ & $4.2$\\
tree & $4.3$ & $4.2$ & $4.5$ & $\mathbf{3.4}$ & $3.7$ & $4.0$ & $4.0$\\
\midrule
avg rank & \bf{3.44} & 3.73 & 4.53 & 3.83 & 3.50 & 4.27 & 4.71\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=mce}
\label{table:mce}
\end{table}

==> tables/results/mlp_dataset_vs_method_conf-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $0.03_{4}$ & $0.03_{3}$ & $\mathbf{0.03_{1}}$ & $0.03_{2}$ & $0.04_{5}$ & $0.04_{6}$ & $0.04_{7}$\\
balance-sc & $\mathbf{0.04_{1}}$ & $0.05_{3}$ & $0.13_{7}$ & $0.05_{2}$ & $0.08_{6}$ & $0.05_{4}$ & $0.08_{5}$\\
car & $\mathbf{0.02_{1}}$ & $0.03_{4}$ & $0.11_{7}$ & $0.03_{2}$ & $0.05_{5}$ & $0.03_{3}$ & $0.08_{6}$\\
cleveland & $0.14_{2}$ & $0.15_{3}$ & $0.19_{7}$ & $\mathbf{0.14_{1}}$ & $0.17_{6}$ & $0.15_{4}$ & $0.17_{5}$\\
dermatolog & $0.04_{4}$ & $0.03_{2}$ & $0.29_{7}$ & $\mathbf{0.03_{1}}$ & $0.09_{6}$ & $0.04_{3}$ & $0.05_{5}$\\
glass & $0.17_{4}$ & $0.17_{3}$ & $0.26_{7}$ & $0.17_{2}$ & $0.18_{5}$ & $0.19_{6}$ & $\mathbf{0.17_{1}}$\\
iris & $0.07_{3}$ & $0.07_{2}$ & $0.22_{7}$ & $\mathbf{0.06_{1}}$ & $0.13_{6}$ & $0.08_{4}$ & $0.12_{5}$\\
landsat-sa & $0.02_{4}$ & $0.02_{3}$ & $0.07_{7}$ & $\mathbf{0.02_{1}}$ & $0.03_{6}$ & $0.02_{5}$ & $0.02_{2}$\\
libras-mov & $0.13_{4}$ & $0.13_{3}$ & $0.50_{7}$ & $\mathbf{0.12_{1}}$ & $0.23_{6}$ & $0.15_{5}$ & $0.12_{2}$\\
mfeat-karh & $0.03_{4}$ & $0.02_{2}$ & $0.16_{7}$ & $\mathbf{0.02_{1}}$ & $0.05_{6}$ & $0.03_{5}$ & $0.03_{3}$\\
mfeat-morp & $0.05_{2}$ & $\mathbf{0.05_{1}}$ & $0.13_{7}$ & $0.05_{5}$ & $0.06_{6}$ & $0.05_{3}$ & $0.05_{4}$\\
mfeat-zern & $0.05_{2}$ & $0.05_{3}$ & $0.14_{7}$ & $\mathbf{0.04_{1}}$ & $0.07_{5}$ & $0.07_{4}$ & $0.08_{6}$\\
optdigits & $0.01_{5}$ & $0.01_{3}$ & $0.10_{7}$ & $\mathbf{0.01_{1}}$ & $0.02_{6}$ & $0.01_{4}$ & $0.01_{2}$\\
page-block & $0.01_{4}$ & $0.01_{3}$ & $0.06_{7}$ & $\mathbf{0.01_{1}}$ & $0.02_{6}$ & $0.01_{5}$ & $0.01_{2}$\\
pendigits & $0.01_{5}$ & $0.00_{2}$ & $0.07_{7}$ & $\mathbf{0.00_{1}}$ & $0.01_{6}$ & $0.01_{4}$ & $0.00_{3}$\\
segment & $0.02_{4}$ & $0.02_{2}$ & $0.16_{7}$ & $\mathbf{0.02_{1}}$ & $0.03_{6}$ & $0.02_{3}$ & $0.03_{5}$\\
vehicle & $0.06_{3}$ & $0.06_{2}$ & $0.12_{7}$ & $\mathbf{0.06_{1}}$ & $0.08_{6}$ & $0.07_{4}$ & $0.07_{5}$\\
vowel & $0.07_{4}$ & $0.07_{2}$ & $0.31_{7}$ & $\mathbf{0.07_{1}}$ & $0.11_{5}$ & $0.07_{3}$ & $0.16_{6}$\\
waveform-5 & $0.03_{3}$ & $0.03_{4}$ & $0.05_{5}$ & $\mathbf{0.03_{1}}$ & $0.05_{6}$ & $0.03_{2}$ & $0.07_{7}$\\
yeast & $0.08_{6}$ & $0.08_{4}$ & $0.12_{7}$ & $\mathbf{0.07_{1}}$ & $0.08_{5}$ & $0.07_{3}$ & $0.07_{2}$\\
\midrule
avg rank & 3.45 & 2.70 & 6.60 & \bf{1.40} & 5.70 & 4.00 & 4.15\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier mlp with the measure=conf-ece(Friedman statistic test = 7.90E+01, p-value = 5.85E-15)}
\label{table:mlp:conf-ece}
\end{table}


==> tables/results/mlp_dataset_vs_method_cw-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $\mathbf{0.09_{1}}$ & $0.09_{2}$ & $0.10_{4}$ & $0.10_{5}$ & $0.10_{3}$ & $0.11_{6}$ & $0.11_{7}$\\
balance-sc & $0.12_{2}$ & $0.13_{3}$ & $0.29_{7}$ & $\mathbf{0.12_{1}}$ & $0.17_{5}$ & $0.15_{4}$ & $0.20_{6}$\\
car & $\mathbf{0.08_{1}}$ & $0.09_{3}$ & $0.25_{7}$ & $0.09_{2}$ & $0.12_{5}$ & $0.11_{4}$ & $0.19_{6}$\\
cleveland & $\mathbf{0.39_{1}}$ & $0.40_{2}$ & $0.45_{4}$ & $0.43_{3}$ & $0.46_{5}$ & $0.47_{6}$ & $0.49_{7}$\\
dermatolog & $0.10_{4}$ & $0.09_{3}$ & $0.64_{7}$ & $\mathbf{0.08_{1}}$ & $0.21_{6}$ & $0.09_{2}$ & $0.12_{5}$\\
glass & $0.52_{5}$ & $\mathbf{0.48_{1}}$ & $0.68_{7}$ & $0.51_{3}$ & $0.54_{6}$ & $0.52_{4}$ & $0.51_{2}$\\
iris & $0.15_{2}$ & $0.15_{3}$ & $0.47_{7}$ & $\mathbf{0.14_{1}}$ & $0.30_{6}$ & $0.18_{4}$ & $0.29_{5}$\\
landsat-sa & $0.07_{4}$ & $0.07_{3}$ & $0.17_{7}$ & $\mathbf{0.07_{1}}$ & $0.08_{6}$ & $0.08_{5}$ & $0.07_{2}$\\
libras-mov & $0.59_{4}$ & $0.53_{3}$ & $1.20_{7}$ & $\mathbf{0.50_{1}}$ & $0.70_{6}$ & $0.59_{5}$ & $0.52_{2}$\\
mfeat-karh & $0.11_{4}$ & $0.10_{2}$ & $0.36_{7}$ & $\mathbf{0.10_{1}}$ & $0.14_{6}$ & $0.11_{5}$ & $0.10_{3}$\\
mfeat-morp & $0.20_{2}$ & $\mathbf{0.20_{1}}$ & $0.35_{7}$ & $0.20_{3}$ & $0.21_{6}$ & $0.21_{4}$ & $0.21_{5}$\\
mfeat-zern & $0.17_{2}$ & $0.17_{3}$ & $0.38_{7}$ & $\mathbf{0.16_{1}}$ & $0.22_{4}$ & $0.24_{6}$ & $0.23_{5}$\\
optdigits & $0.05_{5}$ & $0.04_{2}$ & $0.21_{7}$ & $\mathbf{0.04_{1}}$ & $0.05_{6}$ & $0.04_{4}$ & $0.04_{3}$\\
page-block & $0.04_{4}$ & $0.04_{2}$ & $0.13_{7}$ & $\mathbf{0.04_{1}}$ & $0.05_{6}$ & $0.04_{5}$ & $0.04_{3}$\\
pendigits & $0.02_{5}$ & $0.02_{2}$ & $0.14_{7}$ & $\mathbf{0.02_{1}}$ & $0.02_{6}$ & $0.02_{4}$ & $0.02_{3}$\\
segment & $0.07_{4}$ & $0.06_{2}$ & $0.34_{7}$ & $\mathbf{0.06_{1}}$ & $0.09_{6}$ & $0.07_{3}$ & $0.08_{5}$\\
vehicle & $0.19_{2}$ & $0.19_{3}$ & $0.33_{7}$ & $\mathbf{0.19_{1}}$ & $0.23_{6}$ & $0.20_{4}$ & $0.21_{5}$\\
vowel & $\mathbf{0.28_{1}}$ & $0.30_{3}$ & $0.73_{7}$ & $0.28_{2}$ & $0.38_{5}$ & $0.31_{4}$ & $0.43_{6}$\\
waveform-5 & $0.09_{4}$ & $0.09_{2}$ & $0.12_{5}$ & $\mathbf{0.09_{1}}$ & $0.14_{6}$ & $0.09_{3}$ & $0.16_{7}$\\
yeast & $0.26_{2}$ & $\mathbf{0.26_{1}}$ & $0.38_{7}$ & $0.27_{3}$ & $0.29_{6}$ & $0.28_{5}$ & $0.28_{4}$\\
\midrule
avg rank & 2.95 & 2.30 & 6.60 & \bf{1.70} & 5.55 & 4.35 & 4.55\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier mlp with the measure=cw-ece(Friedman statistic test = 8.09E+01, p-value = 2.36E-15)}
\label{table:mlp:cw-ece}
\end{table}


==> tables/results/mlp_dataset_vs_method_p-conf-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $0.54_{4}$ & $0.55_{3}$ & $\mathbf{0.61_{1}}$ & $0.59_{2}$ & $0.47_{5}$ & $0.40_{6}$ & $0.36_{7}$\\
balance-sc & $0.32_{4}$ & $\mathbf{0.44_{1}}$ & $0.00_{7}$ & $0.39_{3}$ & $0.11_{6}$ & $0.43_{2}$ & $0.17_{5}$\\
car & $0.49_{2}$ & $0.41_{4}$ & $0.00_{7}$ & $0.48_{3}$ & $0.11_{5}$ & $\mathbf{0.54_{1}}$ & $0.00_{6}$\\
cleveland & $\mathbf{0.52_{1}}$ & $0.45_{4}$ & $0.14_{7}$ & $0.52_{2}$ & $0.27_{5}$ & $0.47_{3}$ & $0.24_{6}$\\
dermatolog & $0.48_{3}$ & $\mathbf{0.51_{1}}$ & $0.00_{7}$ & $0.45_{4}$ & $0.07_{6}$ & $0.41_{5}$ & $0.49_{2}$\\
glass & $\mathbf{0.42_{1}}$ & $0.38_{4}$ & $0.07_{7}$ & $0.38_{3}$ & $0.37_{5}$ & $0.30_{6}$ & $0.42_{2}$\\
iris & $0.51_{3}$ & $0.44_{4}$ & $0.08_{7}$ & $0.35_{5}$ & $0.25_{6}$ & $\mathbf{0.56_{1}}$ & $0.52_{2}$\\
landsat-sa & $0.44_{4}$ & $0.46_{2}$ & $0.00_{7}$ & $\mathbf{0.53_{1}}$ & $0.12_{6}$ & $0.35_{5}$ & $0.45_{3}$\\
libras-mov & $0.40_{3}$ & $0.37_{4}$ & $0.00_{7}$ & $\mathbf{0.42_{1}}$ & $0.01_{6}$ & $0.28_{5}$ & $0.42_{2}$\\
mfeat-karh & $0.32_{4}$ & $0.45_{2}$ & $0.00_{7}$ & $\mathbf{0.58_{1}}$ & $0.03_{6}$ & $0.28_{5}$ & $0.43_{3}$\\
mfeat-morp & $0.46_{3}$ & $\mathbf{0.52_{1}}$ & $0.00_{7}$ & $0.38_{5}$ & $0.19_{6}$ & $0.46_{2}$ & $0.38_{4}$\\
mfeat-zern & $0.24_{3}$ & $0.25_{2}$ & $0.00_{7}$ & $\mathbf{0.37_{1}}$ & $0.01_{5}$ & $0.04_{4}$ & $0.00_{6}$\\
optdigits & $0.23_{5}$ & $0.42_{2}$ & $0.00_{7}$ & $0.38_{3}$ & $0.03_{6}$ & $0.33_{4}$ & $\mathbf{0.44_{1}}$\\
page-block & $0.42_{3}$ & $0.39_{4}$ & $0.00_{7}$ & $\mathbf{0.51_{1}}$ & $0.17_{6}$ & $0.38_{5}$ & $0.43_{2}$\\
pendigits & $0.13_{5}$ & $0.34_{2}$ & $0.00_{7}$ & $\mathbf{0.43_{1}}$ & $0.02_{6}$ & $0.16_{4}$ & $0.27_{3}$\\
segment & $0.35_{4}$ & $0.35_{3}$ & $0.00_{7}$ & $\mathbf{0.46_{1}}$ & $0.08_{6}$ & $0.42_{2}$ & $0.24_{5}$\\
vehicle & $0.44_{4}$ & $0.46_{3}$ & $0.06_{7}$ & $\mathbf{0.49_{1}}$ & $0.27_{6}$ & $0.47_{2}$ & $0.40_{5}$\\
vowel & $0.18_{4}$ & $\mathbf{0.34_{1}}$ & $0.00_{7}$ & $0.29_{3}$ & $0.03_{5}$ & $0.34_{2}$ & $0.00_{6}$\\
waveform-5 & $0.22_{3}$ & $0.21_{4}$ & $0.05_{5}$ & $\mathbf{0.29_{1}}$ & $0.01_{6}$ & $0.23_{2}$ & $0.00_{7}$\\
yeast & $0.31_{5}$ & $0.32_{4}$ & $0.05_{7}$ & $0.41_{2}$ & $0.29_{6}$ & $0.39_{3}$ & $\mathbf{0.41_{1}}$\\
\midrule
avg rank & 3.40 & 2.75 & 6.60 & \bf{2.20} & 5.70 & 3.45 & 3.90\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier mlp with the measure=p-conf-ece(Friedman statistic test = 6.48E+01, p-value = 4.69E-12)}
\label{table:mlp:p-conf-ece}
\end{table}


==> tables/results/mlp_dataset_vs_method_p-cw-ece.tex <==
\begin{table}[tph]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & Dirichlet\_L2 & OvR\_Beta & OvR\_Freq\_Bin & OvR\_Isotonic & OvR\_Width\_Bin & Temp\_Scaling & Uncalibrated\\
\midrule
abalone & $\mathbf{0.67_{1}}$ & $0.64_{2}$ & $0.57_{4}$ & $0.54_{5}$ & $0.60_{3}$ & $0.50_{7}$ & $0.50_{6}$\\
balance-sc & $0.32_{3}$ & $0.39_{2}$ & $0.00_{7}$ & $\mathbf{0.43_{1}}$ & $0.26_{4}$ & $0.09_{6}$ & $0.09_{5}$\\
car & $\mathbf{0.61_{1}}$ & $0.44_{2}$ & $0.00_{7}$ & $0.39_{3}$ & $0.17_{5}$ & $0.23_{4}$ & $0.00_{6}$\\
cleveland & $0.59_{2}$ & $\mathbf{0.61_{1}}$ & $0.40_{5}$ & $0.49_{4}$ & $0.40_{6}$ & $0.52_{3}$ & $0.29_{7}$\\
dermatolog & $0.59_{2}$ & $0.46_{4}$ & $0.00_{7}$ & $0.42_{5}$ & $0.34_{6}$ & $0.50_{3}$ & $\mathbf{0.78_{1}}$\\
glass & $0.57_{4}$ & $0.57_{3}$ & $0.13_{7}$ & $0.37_{6}$ & $0.57_{5}$ & $\mathbf{0.58_{1}}$ & $0.58_{2}$\\
iris & $0.54_{3}$ & $0.41_{5}$ & $0.14_{7}$ & $0.39_{6}$ & $0.50_{4}$ & $0.61_{2}$ & $\mathbf{0.73_{1}}$\\
landsat-sa & $0.33_{3}$ & $0.35_{2}$ & $0.00_{7}$ & $\mathbf{0.44_{1}}$ & $0.12_{6}$ & $0.33_{4}$ & $0.32_{5}$\\
libras-mov & $0.73_{2}$ & $0.57_{4}$ & $0.00_{7}$ & $0.47_{5}$ & $0.34_{6}$ & $\mathbf{0.77_{1}}$ & $0.65_{3}$\\
mfeat-karh & $0.76_{2}$ & $0.68_{4}$ & $0.00_{7}$ & $0.54_{5}$ & $0.43_{6}$ & $\mathbf{0.79_{1}}$ & $0.75_{3}$\\
mfeat-morp & $0.49_{2}$ & $\mathbf{0.50_{1}}$ & $0.00_{7}$ & $0.33_{6}$ & $0.41_{5}$ & $0.45_{3}$ & $0.45_{4}$\\
mfeat-zern & $\mathbf{0.65_{1}}$ & $0.44_{2}$ & $0.00_{7}$ & $0.39_{3}$ & $0.05_{4}$ & $0.03_{5}$ & $0.00_{6}$\\
optdigits & $0.64_{2}$ & $0.58_{4}$ & $0.00_{7}$ & $0.45_{5}$ & $0.43_{6}$ & $\mathbf{0.68_{1}}$ & $0.63_{3}$\\
page-block & $0.31_{2}$ & $0.31_{3}$ & $0.00_{7}$ & $\mathbf{0.35_{1}}$ & $0.24_{4}$ & $0.22_{6}$ & $0.23_{5}$\\
pendigits & $0.56_{3}$ & $0.55_{4}$ & $0.00_{7}$ & $0.49_{5}$ & $0.27_{6}$ & $0.61_{2}$ & $\mathbf{0.69_{1}}$\\
segment & $0.42_{2}$ & $0.42_{3}$ & $0.00_{7}$ & $0.38_{4}$ & $0.22_{6}$ & $\mathbf{0.45_{1}}$ & $0.31_{5}$\\
vehicle & $0.53_{3}$ & $0.53_{4}$ & $0.04_{7}$ & $0.46_{5}$ & $0.28_{6}$ & $0.54_{2}$ & $\mathbf{0.58_{1}}$\\
vowel & $\mathbf{0.83_{1}}$ & $0.63_{3}$ & $0.00_{7}$ & $0.56_{4}$ & $0.30_{5}$ & $0.68_{2}$ & $0.22_{6}$\\
waveform-5 & $0.25_{3}$ & $0.22_{4}$ & $0.03_{5}$ & $\mathbf{0.28_{1}}$ & $0.00_{6}$ & $0.25_{2}$ & $0.00_{7}$\\
yeast & $0.65_{2}$ & $\mathbf{0.66_{1}}$ & $0.01_{7}$ & $0.52_{4}$ & $0.44_{6}$ & $0.52_{3}$ & $0.47_{5}$\\
\midrule
avg rank & \bf{2.20} & 2.90 & 6.65 & 3.95 & 5.25 & 2.95 & 4.10\\
\bottomrule
\end{tabular}
\normalsize
\caption{Ranking of calibration methods applied on the classifier mlp with the measure=p-cw-ece(Friedman statistic test = 6.06E+01, p-value = 3.33E-11)}
\label{table:mlp:p-cw-ece}
\end{table}


==> tables/results/p-conf-ece_rankings.tex <==
\begin{table}[tph]
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=p-conf-ece}
\label{table:p-conf-ece}
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{1.8}$ & $2.9$ & $4.3$ & $3.1$ & $4.4$ & $5.6$ & $5.7$\\
forest & $3.7$ & $2.2$ & $6.0$ & $\mathbf{1.9}$ & $4.7$ & $4.7$ & $4.9$\\
knn & $\mathbf{2.6}$ & $2.6$ & $5.7$ & $2.9$ & $5.1$ & $4.5$ & $4.6$\\
lda & $\mathbf{1.9}$ & $3.0$ & $6.1$ & $2.2$ & $3.9$ & $5.3$ & $5.5$\\
logistic & $2.6$ & $2.9$ & $6.3$ & $\mathbf{1.8}$ & $4.7$ & $3.7$ & $6.0$\\
mlp & $3.4$ & $2.8$ & $6.6$ & $\mathbf{2.2}$ & $5.7$ & $3.5$ & $3.9$\\
nbayes & $\mathbf{2.1}$ & $2.7$ & $5.2$ & $2.5$ & $4.5$ & $4.9$ & $6.1$\\
qda & $3.0$ & $2.1$ & $6.5$ & $\mathbf{2.1}$ & $4.6$ & $4.6$ & $5.2$\\
svc-linear & $2.5$ & $3.0$ & $6.6$ & $\mathbf{2.4}$ & $5.0$ & $3.3$ & $5.1$\\
svc-rbf & $3.4$ & $3.4$ & $6.3$ & $3.0$ & $5.0$ & $\mathbf{2.8}$ & $4.2$\\
tree & $\mathbf{2.5}$ & $3.7$ & $6.4$ & $4.3$ & $5.7$ & $2.6$ & $2.7$\\
\midrule
avg rank & 2.69 & 2.87 & 6.00 & \bf{2.58} & 4.85 & 4.11 & 4.90\\
\bottomrule
\end{tabular}
\end{table}

==> tables/results/p-cw-ece_rankings.tex <==
\begin{table}[tph]
\normalsize
\caption{Ranking of calibration methods applied to each classifier with the measure=p-cw-ece}
\label{table:p-cw-ece}
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lccccccc}
\toprule
 & DirL2 & Beta & FreqB & Isot & WidB & TempS & Uncal\\
\midrule
adas & $\mathbf{2.4}$ & $3.2$ & $4.1$ & $4.2$ & $3.9$ & $5.0$ & $5.2$\\
forest & $3.5$ & $\mathbf{2.3}$ & $5.7$ & $3.0$ & $3.6$ & $5.0$ & $5.0$\\
knn & $2.5$ & $4.0$ & $4.5$ & $\mathbf{2.1}$ & $3.2$ & $5.8$ & $6.0$\\
lda & $\mathbf{1.9}$ & $3.1$ & $5.8$ & $3.0$ & $3.5$ & $5.0$ & $5.8$\\
logistic & $\mathbf{2.2}$ & $2.8$ & $6.4$ & $3.0$ & $4.2$ & $3.9$ & $5.5$\\
mlp & $\mathbf{2.2}$ & $2.9$ & $6.7$ & $4.0$ & $5.2$ & $3.0$ & $4.1$\\
nbayes & $\mathbf{1.4}$ & $3.6$ & $4.8$ & $2.6$ & $4.2$ & $5.3$ & $6.1$\\
qda & $\mathbf{2.2}$ & $2.8$ & $6.3$ & $2.5$ & $3.8$ & $4.8$ & $5.6$\\
svc-linear & $\mathbf{2.3}$ & $2.7$ & $6.7$ & $3.8$ & $4.0$ & $3.7$ & $4.8$\\
svc-rbf & $\mathbf{2.9}$ & $3.0$ & $6.3$ & $3.5$ & $4.1$ & $3.9$ & $4.3$\\
tree & $\mathbf{2.4}$ & $4.3$ & $5.9$ & $4.2$ & $5.2$ & $3.0$ & $3.0$\\
\midrule
avg rank & \bf{2.34} & 3.15 & 5.73 & 3.27 & 4.11 & 4.37 & 5.02\\
\bottomrule
\end{tabular}
\end{table}

==> tables/results_dnn/rankings_duo_ECE_cw_ECE.tex <==
\begin{table}
\begin{minipage}[t]{.44\textwidth}
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lcccccc}
\toprule
 &  uncal &  temp\_s &  vec\_s &  dir\_diag &  dir\_off &  mat\_off \\
\midrule
densenet40\_c10      & $0.06_{6}$ & $\mathbf{0.01_{1}}$ & $0.01_{3}$ & $0.01_{5}$ & $0.01_{4}$ & $0.01_{2}$ \\
densenet40\_c100     & $0.21_{6}$ & $\mathbf{0.01_{1}}$ & $0.01_{4}$ & $0.01_{3}$ & $0.01_{2}$ & $0.02_{5}$ \\
lenet5\_c10          & $0.05_{6}$ & $0.02_{5}$ & $\mathbf{0.01_{1}}$ & $0.01_{3}$ & $0.01_{2}$ & $0.01_{4}$ \\
lenet5\_c100         & $0.12_{6}$ & $0.01_{3}$ & $\mathbf{0.01_{1}}$ & $0.02_{4}$ & $0.02_{5}$ & $0.01_{2}$ \\
pretrained\_c10      & $0.05_{6}$ & $0.01_{5}$ & $\mathbf{0.01_{1}}$ & $0.01_{3}$ & $0.01_{4}$ & $0.01_{2}$ \\
pretrained\_c100     & $0.18_{6}$ & $0.01_{2}$ & $0.02_{3}$ & $\mathbf{0.01_{1}}$ & $0.02_{4}$ & $0.03_{5}$ \\
pretrained\_mnist    & $0.01_{6}$ & $\mathbf{0.00_{1}}$ & $0.00_{2}$ & $0.01_{5}$ & $0.00_{3}$ & $0.00_{4}$ \\
pretrained\_svhn     & $0.08_{6}$ & $0.01_{5}$ & $0.01_{2}$ & $\mathbf{0.01_{1}}$ & $0.01_{3}$ & $0.01_{4}$ \\
resnet110\_SD\_c10    & $0.04_{6}$ & $\mathbf{0.01_{1}}$ & $0.01_{3}$ & $0.01_{5}$ & $0.01_{4}$ & $0.01_{2}$ \\
resnet110\_SD\_c100   & $0.16_{6}$ & $\mathbf{0.01_{1}}$ & $0.01_{2}$ & $0.02_{3}$ & $0.02_{5}$ & $0.02_{4}$ \\
resnet110\_c10       & $0.05_{6}$ & $0.01_{4}$ & $0.01_{3}$ & $0.01_{5}$ & $0.01_{2}$ & $\mathbf{0.01_{1}}$ \\
resnet110\_c100      & $0.18_{6}$ & $\mathbf{0.02_{1}}$ & $0.03_{2}$ & $0.03_{3}$ & $0.03_{5}$ & $0.03_{4}$ \\
resnet152\_SD\_SVHN   & $0.01_{6}$ & $0.01_{4}$ & $0.01_{2}$ & $0.01_{5}$ & $\mathbf{0.01_{1}}$ & $0.01_{3}$ \\
resnet\_wide32\_c10   & $0.05_{6}$ & $0.01_{4}$ & $0.01_{3}$ & $\mathbf{0.01_{1}}$ & $0.01_{5}$ & $0.01_{2}$ \\
resnet\_wide32\_c100  & $0.19_{6}$ & $\mathbf{0.01_{1}}$ & $0.02_{2}$ & $0.02_{3}$ & $0.02_{4}$ & $0.03_{5}$ \\
\midrule  
 avg rank & 6.0 & 2.6 & 2.27 & 3.33 & 3.53 & 3.27\\
\bottomrule
\end{tabular}
\normalsize
\captionof{table}{ECE.}
\label{table:res:ece}
\end{minipage}
\hfill
\begin{minipage}[t]{.44\textwidth}
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{cccccc}
\toprule
 uncal &  temp\_s &  vec\_s &  dir\_diag &  dir\_off &  mat\_off \\
\midrule
$0.11_{6}$ & $0.04_{5}$ & $\mathbf{0.04_{1}}$ & $0.04_{4}$ & $0.04_{3}$ & $0.04_{2}$ \\
$0.47_{6}$ & $0.19_{3}$ & $0.19_{4}$ & $\mathbf{0.19_{1}}$ & $0.19_{2}$ & $0.19_{5}$ \\
$0.20_{6}$ & $0.17_{5}$ & $0.06_{2}$ & $\mathbf{0.06_{1}}$ & $0.06_{4}$ & $0.06_{3}$ \\
$0.47_{6}$ & $0.38_{5}$ & $\mathbf{0.20_{1}}$ & $0.22_{4}$ & $0.21_{2}$ & $0.21_{3}$ \\
$0.10_{6}$ & $0.04_{4}$ & $0.04_{2}$ & $\mathbf{0.04_{1}}$ & $0.05_{5}$ & $0.04_{3}$ \\
$0.42_{6}$ & $\mathbf{0.23_{1}}$ & $0.24_{5}$ & $0.24_{3}$ & $0.24_{4}$ & $0.24_{2}$ \\
$0.02_{4}$ & $\mathbf{0.02_{1}}$ & $0.02_{2}$ & $0.03_{6}$ & $0.02_{5}$ & $0.02_{3}$ \\
$0.16_{6}$ & $0.04_{5}$ & $0.02_{2}$ & $\mathbf{0.02_{1}}$ & $0.03_{3}$ & $0.03_{4}$ \\
$0.09_{6}$ & $0.03_{4}$ & $0.03_{2}$ & $0.03_{5}$ & $0.03_{3}$ & $\mathbf{0.03_{1}}$ \\
$0.38_{6}$ & $0.20_{5}$ & $\mathbf{0.17_{1}}$ & $0.18_{2}$ & $0.19_{4}$ & $0.19_{3}$ \\
$0.10_{6}$ & $0.04_{5}$ & $0.04_{2}$ & $0.04_{3}$ & $0.04_{4}$ & $\mathbf{0.04_{1}}$ \\
$0.42_{6}$ & $0.20_{4}$ & $0.19_{3}$ & $0.19_{2}$ & $\mathbf{0.19_{1}}$ & $0.20_{5}$ \\
$0.02_{2}$ & $\mathbf{0.02_{1}}$ & $0.02_{5}$ & $0.02_{6}$ & $0.02_{3}$ & $0.02_{4}$ \\
$0.10_{6}$ & $0.05_{5}$ & $0.03_{4}$ & $\mathbf{0.03_{1}}$ & $0.03_{3}$ & $0.03_{2}$ \\
$0.42_{6}$ & $0.19_{5}$ & $\mathbf{0.17_{1}}$ & $0.18_{2}$ & $0.18_{3}$ & $0.18_{4}$ \\
\midrule 
5.6 & 3.87 & 2.47 & 2.8 & 3.27 & 3.0\\
\bottomrule
\end{tabular}
\normalsize
\captionof{table}{classwise-ECE.}
\label{table:res:cw-ece}
\end{minipage}
\end{table}

==> tables/results_dnn/rankings_duo_nll_brier.tex <==
\begin{table}
\begin{minipage}[t]{.44\textwidth}
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{lcccccc}
\toprule
  &   uncal &  temp\_s &  vec\_s &  dir\_diag &  dir\_off &  mat\_off \\
\midrule
densenet40\_c10      & $0.43_{6}$ & $0.23_{5}$ & $0.22_{2}$ & $0.22_{4}$ & $0.22_{3}$ & $\mathbf{0.22_{1}}$ \\
densenet40\_c100     & $2.02_{6}$ & $1.06_{2}$ & $1.06_{3}$ & $1.06_{5}$ & $1.06_{4}$ & $\mathbf{1.05_{1}}$ \\
lenet5\_c10          & $0.82_{6}$ & $0.80_{5}$ & $0.75_{3}$ & $0.75_{4}$ & $0.74_{2}$ & $\mathbf{0.74_{1}}$ \\
lenet5\_c100         & $2.78_{6}$ & $2.65_{5}$ & $2.52_{3}$ & $2.52_{4}$ & $2.49_{2}$ & $\mathbf{2.49_{1}}$ \\
pretrained\_c10      & $0.39_{6}$ & $\mathbf{0.19_{1}}$ & $0.20_{5}$ & $0.20_{3}$ & $0.20_{2}$ & $0.20_{4}$ \\
pretrained\_c100     & $1.64_{6}$ & $\mathbf{0.94_{1}}$ & $0.96_{5}$ & $0.96_{4}$ & $0.96_{2}$ & $0.96_{3}$ \\
pretrained\_mnist    & $0.06_{6}$ & $\mathbf{0.05_{1}}$ & $0.06_{4}$ & $0.06_{5}$ & $0.06_{3}$ & $0.06_{2}$ \\
pretrained\_svhn     & $0.20_{6}$ & $0.15_{5}$ & $0.14_{3}$ & $0.15_{4}$ & $0.14_{2}$ & $\mathbf{0.14_{1}}$ \\
resnet110\_SD\_c10    & $0.30_{6}$ & $0.18_{5}$ & $0.18_{2}$ & $0.18_{4}$ & $0.18_{3}$ & $\mathbf{0.18_{1}}$ \\
resnet110\_SD\_c100   & $1.35_{6}$ & $0.94_{4}$ & $\mathbf{0.92_{1}}$ & $0.93_{3}$ & $0.94_{5}$ & $0.93_{2}$ \\
resnet110\_c10       & $0.36_{6}$ & $0.21_{5}$ & $0.21_{3}$ & $0.21_{4}$ & $0.21_{2}$ & $\mathbf{0.20_{1}}$ \\
resnet110\_c100      & $1.69_{6}$ & $1.09_{3}$ & $1.09_{2}$ & $1.09_{4}$ & $1.10_{5}$ & $\mathbf{1.07_{1}}$ \\
resnet152\_SD\_SVHN   & $0.09_{6}$ & $\mathbf{0.08_{1}}$ & $0.08_{4}$ & $0.08_{5}$ & $0.08_{2}$ & $0.08_{3}$ \\
resnet\_wide32\_c10   & $0.38_{6}$ & $0.19_{5}$ & $0.18_{3}$ & $0.18_{4}$ & $0.18_{2}$ & $\mathbf{0.18_{1}}$ \\
resnet\_wide32\_c100  & $1.80_{6}$ & $0.94_{3}$ & $0.94_{2}$ & $0.95_{4}$ & $0.95_{5}$ & $\mathbf{0.93_{1}}$ \\
\midrule 
 avg rank & 6.0 & 3.4 & 3.0 & 4.03 & 2.97 & 1.6\\
\bottomrule
\end{tabular}
\normalsize
\captionof{table}{NLL.}
\label{table:res:nll}
\end{minipage}
\hfill
\begin{minipage}[t]{.44\textwidth}
\tiny
\centering
\setlength{\tabcolsep}{.6em}
\begin{tabular}{cccccc}
\toprule
 uncal &  temp\_s &  vec\_s &  dir\_diag &  dir\_off &  mat\_off \\
\midrule
$0.013_{6}$ & $0.011_{4}$ & $0.011_{3}$ & $0.011_{5}$ & $0.011_{2}$ & $\mathbf{0.011_{1}}$ \\
$0.005_{6}$ & $0.004_{3}$ & $0.004_{5}$ & $0.004_{4}$ & $0.004_{2}$ & $\mathbf{0.004_{1}}$ \\
$0.038_{6}$ & $0.037_{5}$ & $0.035_{4}$ & $0.035_{3}$ & $0.035_{2}$ & $\mathbf{0.035_{1}}$ \\
$0.008_{6}$ & $0.008_{5}$ & $0.008_{4}$ & $0.008_{3}$ & $0.008_{2}$ & $\mathbf{0.008_{1}}$ \\
$0.011_{6}$ & $\mathbf{0.010_{1}}$ & $0.010_{5}$ & $0.010_{4}$ & $0.010_{3}$ & $0.010_{2}$ \\
$0.004_{6}$ & $\mathbf{0.004_{1}}$ & $0.004_{5}$ & $0.004_{3}$ & $0.004_{2}$ & $0.004_{4}$ \\
$0.003_{3}$ & $\mathbf{0.003_{1}}$ & $0.003_{6}$ & $0.003_{5}$ & $0.003_{2}$ & $0.003_{4}$ \\
$0.008_{6}$ & $0.006_{5}$ & $0.006_{3}$ & $0.006_{4}$ & $\mathbf{0.005_{1}}$ & $0.005_{2}$ \\
$0.010_{6}$ & $0.009_{5}$ & $0.009_{2}$ & $0.009_{4}$ & $0.009_{3}$ & $\mathbf{0.009_{1}}$ \\
$0.004_{6}$ & $0.004_{5}$ & $0.004_{2}$ & $\mathbf{0.004_{1}}$ & $0.004_{4}$ & $0.004_{3}$ \\
$0.011_{6}$ & $0.010_{4}$ & $0.010_{3}$ & $0.010_{5}$ & $0.010_{2}$ & $\mathbf{0.010_{1}}$ \\
$0.005_{6}$ & $0.004_{4}$ & $0.004_{5}$ & $0.004_{2}$ & $0.004_{3}$ & $\mathbf{0.004_{1}}$ \\
$0.003_{3}$ & $\mathbf{0.003_{1}}$ & $0.003_{6}$ & $0.003_{4}$ & $0.003_{2}$ & $0.003_{5}$ \\
$0.010_{6}$ & $0.009_{5}$ & $0.009_{4}$ & $0.009_{2}$ & $\mathbf{0.009_{1}}$ & $0.009_{3}$ \\
$0.004_{6}$ & $0.004_{5}$ & $0.004_{3}$ & $0.004_{2}$ & $0.004_{4}$ & $\mathbf{0.004_{1}}$ \\
\midrule 
 5.6 & 3.6 & 4.0 & 3.4 & 2.33 & 2.07\\
\bottomrule
\end{tabular}
\normalsize
\captionof{table}{Brier Score.}
\label{table:res:brier}
\end{minipage}
\end{table}
